Multivariate Density Estimation via Variance-Reduced Sketching

Multivariate density estimation is of great interest in various scientific and engineering disciplines. In this work, we introduce a new framework called Variance-Reduced Sketching (VRS), specifically designed to estimate multivariate density functions with a reduced curse of dimensionality. Our VRS framework conceptualizes multivariate functions as infinite-size matrices/tensors, and facilitates a new sketching technique motivated by the numerical linear algebra literature to reduce the variance in density estimation problems. We demonstrate the robust numerical performance of VRS through a series of simulated experiments and real-world data applications. Notably, VRS shows remarkable improvement over existing neural network density estimators and classical kernel methods in numerous distribution models. Additionally, we offer theoretical justifications for VRS to support its ability to deliver density estimation with a reduced curse of dimensionality.

==> test.tex <==

 
\begin{lemma} \label{lemma:sobolev matrix Bernstein} Suppose  $\{ \BZ_i\}_{i=1}^N  $ are i.i.d. data  sampled from  the density $A^*$ and  $\widehat A =\frac{1}{N}\sum_{i=1}^N \delta_{\BZ_i}$ are the corresponding empirical measure.    Let $p  \in \mathbb Z^+$ be such that $p< d$.
Suppose  $\{\phi_k \}_{k=1}^{\infty } $ be a collection of $ \lt([0,1])$ basis such that $\|\phi_k \|_\infty \le C_{\phi} $ for some absolute constant $C_{\phi} $.
For positive integers $\m$ and $\l$, denote  
\begin{align} \label{eq:projection basis 1}
\mathcal M =\Span \bigg\{\phi_{\mi_1}(z_1)  \cdots  \phi_{\mi_{p}}(z_{p}) \bigg \}_{\mi_1, \ldots, \mi_{p}=1}^\m \  \text{and} \ \   
\mathcal N = \Span\bigg\{  \phi_{\li_1 }(z_{p+1})\cdots  \phi_{\li_{{d-p}}}(z_{d })\bigg\}_{\li_1, \ldots, \li_{{d-p} }=1}^\l.
\end{align} 
Suppose in addition that $ N \ge C_1  \max\{ m^{p}, l^{{d-p}}\}    $ for some absolute constant $C_1$. Then it holds that
$$\|  (\widehat A - A ^*) \times_x \mathcal P_\mathcal M \times_y \mathcal P_{\mathcal N}  \|_{\op}  ={\bigO}_{ \mathbb P} \bigg(\sqrt{ \frac{\m^{p} +\l^{{d-p}}}{N}}   \bigg) . $$

\end{lemma} 
 \begin{proof}
 Denote  
$$x=(z_1,\ldots, z_{p}) \quad \text{and} \quad  y=(z_{p+1},\ldots,  z_{d}).$$
For positive integers $\m$ and $\l$, by ordering the indexes $(\mi_1,\ldots, \mi_{p})$ and  $(\li_1,\ldots, \li_{{d-p}})$   in \eqref{eq:projection basis 1}, we can also write
 \begin{align} %\label{eq:projection basis for x and y 2}
 \mathcal M =\text{span}\{\Phi_\mi(x) \}_{\mi=1}^{\m^{p}}  \quad \text{and} \quad 
 \mathcal N =  \text{span} \{  \Psi_{\li }(y )  \}_{\li =1}^{\l^{{d-p}}}.
 \end{align}  
Note that $   \widehat  A   \times_x \mathcal P_\mathcal M \times_y \mathcal P_{\mathcal N}  $
and $   A ^*  \times_x \mathcal P_\mathcal M \times_y \mathcal P_{\mathcal N} $ are both zero outsize the subspace $\mathcal M\otimes \mathcal N $. Recall $\{Z_i\}_{i=1}^N \subset [0,1]^d$ are independently samples forming $\widehat{A }$. Let $\widehat B$ and $B^*$ be two matrices in $\mathbb R^{\m^{p}\times \l^{{d-p}}}$ such that 
\begin{align*}
\widehat B_{\mi,\li}= \widehat A [ \Phi_\mi, \Psi_\li] = \frac{1}{N}\sum_{i=1}^N \Phi_\mi(X_i)  \Psi_\li(Y_i)  \quad \text{and} \quad  B_{\mi,\li}^*=   A^*[ \Phi_\mi, \Psi_\li] =\E(\widehat A [ \Phi_\mi, \Psi_\li])  ,
\end{align*}
where $X_i=(Z_{i,1},\ldots, Z_{i,p})  \in \mathbb R^{p}$ and $Y_i=(Z_{i,p+1}, \ldots, Z_{i, d})   \in \mathbb R^{{d-p}}$. Note that  
\begin{align} %\label{eq:matrix bernstein in hilbert space}
\| \widehat B -B ^* \|_{\op} = \|  (\widehat A  - A  ^*) \times_x \mathcal P_\mathcal M \times_y \mathcal P_{\mathcal N}  \|_{\op}. 
\end{align}
\
\\  
{\bf Step 1.} Let $v= (v_1,\ldots, v_{\m^{p} })  \in \mathbb R^{\m^{p} }$ and suppose that 
$\|v\|_2=1 $.
Then by orthonormality of $  \{\Phi_{\mi }(x)     \}_{\mi=1 }^{\m^{p}}$ in $\lt ([0,1]^{p}) $ it follows that 
$$\bigg\| \sum_{\mi=1}^{\m^{p}}  v_\mi \Phi_\mi \bigg\|_{\lt([0,1]^{p})} ^2 =1. $$
%\red{wait tomorrow continue}
In addition, since 
$$\| \phi_{\mi_1 }(z_1)\cdots \phi_{\mi_{p}  }(z_{p})  \|_\infty \le \prod_{j=1}^{p}\|\phi_{\mi_j } \|_\infty  \le C_{\phi}^{p},   $$   it follows that   
$\|\Phi_\mi \|_\infty \le C_{\phi}^{p} $ for all $1\le \mi\le \m^{p}$ and 
$$ \bigg\| \sum_{\mi=1}^{\m^{p}}  v_{\mi} \Phi_{\mi} \bigg\|_\infty   \le 
 \sqrt{ \sum_{\mi=1}^{\m^{p}} v_{\mi}^2 } \sqrt{\sum_{\mi=1}^{\m^{p}}  \|   \Phi_{\mi}  \|_\infty ^2  } =O(\sqrt {\m^{p}}). $$
\\
\\
{\bf Step 2.}   Let $w= (w_1,\ldots, w_{\l^{{d-p}}})  \in \mathbb R^{\l^{{d-p}} }$ and suppose that 
$\|w\|_2=1 $. Then by orthonormality of $\{  \Psi_{\li }(y )  \}_{\li=1}^{\l^{{d-p}}}$ in $\lt([0,1]^{{d-p}})$,
$$\bigg\| \sum_{\li=1}^{\l^{{d-p}}} w_{\li} \Psi_{\li} \bigg\|^2_{\lt([0,1]^d)}  =1. $$
In addition, since 
$$\| \phi_{\li_1 }(z_{p+1} )\cdots \phi_{\li_{ {d-p}}  }(z_{d})  \|_\infty \le \prod_{j=1}^{{d-p}}\|\phi_{\li_j } \|_\infty  \le C_{\phi}^{{d-p}},   $$
it follows that 
$ \|  \Psi_{\li } \|_\infty  \le C_{\phi}^{{d-p}}$. Therefore 
$$\bigg\| \sum_{\li=1}^{\l^{{d-p}}} w_{\li} \Psi_{\li} \bigg\|_\infty   \le  \sqrt{ \sum_{\li=1}^{\l^{{d-p}}} w_{\li}^2}  \sqrt {  \sum_{\li=1}^{\l^{{d-p}}}   \| \Psi_{\li}  \|_\infty ^2  }  =O(  \sqrt{\l^{{d-p}}}). $$
\
\\
{\bf Step 3.} For fixed  $v= (v_1,\ldots, v_{\m^{p} }) $ and $ w =(w_1,\ldots, w_{\l^{{d-p}}})    $, we bound 
$ v^\top (B^*- \widehat B) w. $
Let  $ \Delta_i =\sum_{\mi=1}^{\m^{p}}   v_{\mi}     \Phi_{\mi} (X_i)  \sum_{\li=1}^{\l^{{d-p}}} w_{\li} \Psi_{\li} (Y_i) $. Then 
\begin{align*} & Var (\Delta_i  ) \le \E(\Delta_i^2) = \iint  \bigg\{  \sum_{\mi=1}^{\m^{p}}  v_{\mi}     \Phi_{\mi} (x ) \bigg\}^2 \bigg\{  \sum_{\li=1}^{\l^{{d-p}}}  w_{\li}     \Psi_{\li} (y ) \bigg\}^2   A ^*(x,y) \mathrm{d}x\mathrm{d}y  
\\
\le &\|  A  ^*\|_\infty \int  \bigg\{  \sum_{\mi=1}^{\m^{p}}  v_{\mi}     \Phi_{\mi} (x ) \bigg\}^2 \mathrm{d}x \int  \bigg\{  \sum_{\li=1}^{\l^{{d-p}}}  w_{\li}     \Psi_{\li} (y) \bigg\}^2  \mathrm{d}y  
\\
= & \|  A  ^*\|_\infty  \bigg \| \sum_{\mi=1}^{\m^{p}}   v_{\mi}     \Phi_{\mi}  \bigg\|_{\lt([0,1]^{p})}  ^2\bigg \|    \sum_{\li=1}^{\l^{{d-p}}}  w_{\li}     \Psi_{\li}   \bigg\|_{\lt([0,1]^{{d-p}})}  ^2 =\|A ^*\|_\infty .
\end{align*}
where the last  equality follows from {\bf Step 1} and {\bf Step 2}.
In addition,
$$|\Delta_i| \le \|  \sum_{\mi=1}^{\m^{p}}  v_{\mi}     \Phi_{\mi} (X_i)  \|_\infty \|\sum_{\li=1}^{\l^{{d-p}}} w_{\li} \Psi_{\li} (Y_i) \|_\infty =O( \sqrt{\m^{p} \l^{{d-p}}}) .$$
So for given $v, w$, by Bernstein's inequality
\begin{align*} &\p\bigg(  \bigg|  v^\top (B^*-\widehat B) w \bigg| \ge t  \bigg) 
=  \p\bigg(   \bigg| \frac{1}{N} \sum_{i=1}^N \Delta_i -\E(\Delta_i) \bigg| \ge t\bigg) \le 2\exp\bigg ( \frac{-cNt^2 }{\| A ^* \|_\infty + t\sqrt{ \m^{p}  \l^{ {d-p}}} } \bigg) .
\end{align*}
\
\\
{\bf Step 4.}
Let $\mathcal N ( \frac{1}{4},\m^{p})  $ be a $1/4$ covering net of unit ball in $\mathbb R ^{\m^{p}}$ and 
$ \mathcal N( \frac{1}{4},\l^{{d-p}} )$  be a $1/4$ covering net of unit ball in $\mathbb R^{\l^{{d-p}}} $, then by 4.4.3  on page 90 of \cite{vershynin2018high} 
\begin{align*}
  \|    B^* -\widehat B   \|_{\op}  \le  2\sup_{v \in\mathcal N( \frac{1}{4},\m^{p}), w\in \mathcal N( \frac{1}{4},\l^{{d-p}})} v^\top ( B^* -\widehat B ) w.
\end{align*}
So by union bound and the fact that the size of $\mathcal N ( \frac{1}{4},\m^{p})$ is bounded by $9^{\m^{p}}$ and the size of $\mathcal N ( \frac{1}{4},\l^{{d-p}} )$ is bounded by $9^{\l^{{d-p}}}$, 
\begin{align*}
 \p \bigg( \|    B^* -\widehat B   \|_{\op} \ge t \bigg)  
\le  &\p \bigg(   \sup_{v \in\mathcal N( \frac{1}{4},\m^{p}), w\in \mathcal N( \frac{1}{4},\l^{{d-p}})} v^\top ( B^* -\widehat B  ) w \ge  t/2\bigg) 
\\
 \le & 2\cdot 9^{\m^{p} +\l^{{d-p}}}\exp\bigg ( \frac{-cNt^2 }{\|A ^*\|_\infty + t \sqrt{\m^{p}\l^{{d-p}} }} \bigg).
\end{align*}
This implies that 
$$     \|B^* -\widehat B  \|_{\op} =\OP \bigg(\sqrt{ \frac{\m^{p} +\l^{{d-p}}}{N}} + \frac{ \m^{3p/2 } \l^{  {d-p}/2 } + \m^{ p/2 } \l^{  3{d-p}/2 }}{N} \bigg) .$$
%The desired result follows from  \eqref{eq:matrix bernstein in hilbert space}.
\end{proof} 
